From Factor Models to Deep Learning: Machine Learning in Reshaping Empirical Asset Pricing

This paper comprehensively reviews the application of machine learning (ML) and AI in finance, specifically in the context of asset pricing. It starts by summarizing the traditional asset pricing models and examining their limitations in capturing the complexities of financial markets. It explores how 1) ML models, including supervised, unsupervised, semi-supervised, and reinforcement learning, provide versatile frameworks to address these complexities, and 2) the incorporation of advanced ML algorithms into traditional financial models enhances return prediction and portfolio optimization. These methods can adapt to changing market dynamics by modeling structural changes and incorporating heterogeneous data sources, such as text and images. In addition, this paper explores challenges in applying ML in asset pricing, addressing the growing demand for explainability in decision-making and mitigating overfitting in complex models. This paper aims to provide insights into novel methodologies showcasing the potential of ML to reshape the future of quantitative finance.

==> return_prediction.tex <==
\section{Estimating Risk Premia/ Expected Return}
\label{estimatingriskpremia}
Predictive machine learning tasks for asset pricing encompass a range of sophisticated analytical models that significantly enhance financial forecasting. These tasks include asset price and return prediction, where ML algorithms analyze past trends and market data to forecast future values. They also extend to asset movement prediction, enabling the anticipation of price direction changes, and asset ranking prediction, which involves assessing assets based on potential growth or risk. Additionally, in the realm of options trading, ML models are crucial for predicting option pricing and volatility, offering valuable insights for trading strategies. This comprehensive application of ML in asset pricing represents a major leap in financial analysis, providing deeper and more accurate market insights.

\subsection{Asset Price/Return Prediction}
With the rise of deep learning, researchers in the field of return prediction have progressively evolved their methodologies. Initially, simple feedforward models and random forest were employed \cite{singh2017stock,vijh2020stock}, offering a basic approach to stock return prediction. Soon, the focus shifted to Recurrent Neural Networks (RNN) and especially Long-Short Term Memory (LSTM) \cite{khare2017short,pawar2019stock,moghar2020stock}, which were better equipped to capture long-term dependencies in market data, enhancing the accuracy of predictions. 
As understanding deepened, more complex and sophisticated models emerged. TS-Mixer \cite{ye2023prediction} combined long-term and short-term temporal mixers, offering a nuanced approach to capturing both local and global market patterns. In parallel, there was a move towards integrating multiple models to leverage their individual strengths. The CNN-BiLSTM-AM \cite{lu2021cnn} combines Convolutional Neural Networks, Bi-directional Long Short-Term Memory, and Attention Mechanisms. \cite{uddin2021attention} uses attention mechanisms to create dynamic networks that evolve over time, linking various firms and incorporating their accounting fundamentals. GNNs represent a significant leap forward, enabling models to capture complex relationships and interactions within the financial market, leading to more accurate and reliable predictions.

\subsubsection{Evaluation Metrics}
In the field of asset pricing and return prediction, accurately evaluating the performance of predictive models is crucial. Three widely used metrics are:

\textbf{Root Mean Square Error (RMSE)} is particularly valuable as it provides a measure of the standard deviation of the prediction errors, highlighting the average magnitude of errors in a model's predictions. 

\textbf{Mean Absolute Error (MAE)}, on the other hand, offers a straightforward average of absolute errors, giving a clear indication of prediction accuracy without giving undue emphasis to large errors, unlike RMSE. 

\textbf{Mean Absolute Percentage Error (MAPE)} extends this by expressing prediction accuracy as a percentage, making it easier to interpret and compare across different scales of data. Each of these metrics serves a unique purpose in assessing the precision and reliability of models used for forecasting asset prices and returns, offering a comprehensive view of their performance in varying market conditions.






\subsubsection{Evaluation Metrics}
Common evaluation metrics for asset ranking include:

\textbf{Mean Average Precision (MAP)} evaluates the quality of information retrieval systems. It computes the average precision (AP) for each query and then takes the mean of these values over all queries. AP for a single query is the average of the precision values at each relevant item in the retrieval list. A specific variant of MAP that considers only the top K predictions for each query is MAP@K. This can be mathematically represented as:

\begin{equation}
    \text{MAP@K} = \frac{1}{|S|} \sum_{s \in S} \frac{1}{K} \sum_{k=1}^{K} P(k)_s \cdot \text{rel}(k)_s
\end{equation}

Where \( |S| \) denotes the number of samples in the test data.
\( P(k)_s \) is the precision measuring overall hits of the top-K results in the \( s \)-th sample.
\( \text{rel}(k)_s \) is a binary function indicating the relevance of a rank \( k \) in the \( s \)-th sample.

\textbf{Mean Reciprocal Rank (MRR)} measures the reciprocal of the rank position at which the highest-return asset, as per the ground truth, is correctly predicted in the ranking list. This metric is crucial in assessing how well a ranking model can identify and place the most valuable assets at the top of its predictions.

\begin{equation}
\text{MRR} = \frac{1}{|S|} \sum_{s \in S} \frac{1}{\text{rank}_s}
\end{equation}

Where \( |S| \) is the number of samples in the test data, and \( \text{rank}_s \) is the rank of the top-return item in the ground-truth for the \( s \)-th sample.

\textbf{Normalized Discounted Cumulative Gain (NDCG)} is a key metric for evaluating ranking algorithms, particularly in stock ranking. $\text{NDCG@k}$ assesses the quality of predictions for the top $k$ stocks. It is calculated as:

\begin{equation}
\text{NDCG@k} = \sum_{i=1}^{k} \frac{2^{\text{rel}_i} - 1}{\log_2(i+1)}
\end{equation}

In this equation, $\text{rel}_i$ represents the relevance score of the item at rank $i$, and $k$ is the cutoff rank, i.e., the top $k$ stocks. The formula reflects the diminishing importance of items as they appear lower in the ranking.

\subsection{Option Pricing Prediction}
Option pricing prediction is a sophisticated area in financial machine learning, where algorithms are used to forecast the future pricing of options. This task is complex due to the intricate nature of options, which are influenced by various factors including the underlying asset price, volatility, time to expiration, and interest rates. Machine learning models, particularly those leveraging techniques like deep learning and time series analysis, are adept at parsing through these multifaceted variables to predict option prices accurately. This capability is crucial for traders and investors, as it aids in making informed decisions about buying or selling options, assessing their fair value, and managing risk. Accurate option pricing prediction also plays a vital role in developing effective hedging strategies and in overall portfolio optimization, making it a key component in the arsenal of modern financial analytics.

\cite{ivașcu2021option} explore the efficacy of various Machine Learning algorithms in option pricing, particularly for European call options based on WTI crude oil future contracts. It critiques the limitations of classic parametric models, like computational demands and unrealistic assumptions, advocating for a non-parametric, data-driven approach. While previous research predominantly focused on neural networks, this study expands the scope to include Support Vector Regressions, Genetic Algorithms, and three Decision Tree methods: Random Forest, XGBoost, and LightGBM. By comparing these with traditional models like Black-Scholes and Corrado-Su, using both historical and implied parameters, the paper demonstrates the superior performance of Machine Learning algorithms in option pricing. This is evident across various contract moneynesses and maturities, marking a significant contribution to the field of financial modeling and analytics.

\cite{culkin2017machine} use a fully-connected feed-forward neural network to accurately replicate the Black and Scholes option pricing formula. It highlights the potential of deep learning to automate complex financial roles and suggests that such models could learn and mimic the strategies of specialized option pricing traders, demonstrating a significant advancement in the field of financial technology and analysis.

\cite{chowdhury2020predicting} adapt the Black–Scholes Option Pricing Model (BSOPM) to forecast stock prices in frontier markets, specifically focusing on call and put options as proxies for buying and selling prices. It introduces modifications to BSOPM, tailoring it to frontier market conditions by recalibrating parameters like strike price and expiration time. To validate these modifications, the study employs machine learning algorithms, including decision trees, ensemble methods, and neural networks, via Rapidminer software. The findings indicate that machine learning predictions align closely with BSOPM results, but with enhanced accuracy due to machine learning's ability to account for continuously changing risk and dividend parameters. Additionally, the study numerically analyzes volatility and draws parallels between the modified BSOPM and quantum physics concepts, like the Schrodinger and heat equations, offering a novel perspective in financial modeling.
